Continuously Learning Bug Locations

Automatically locating buggy changesets associated with bug reports is crucial in the software development process. Deep Learning (DL)-based techniques show promising results by leveraging structural information from the code and learning links between changesets and bug reports. However, since source code associated with changesets evolves, the performance of such models tends to degrade over time due to concept drift. Aiming to address this challenge, in this paper, we evaluate the potential of using Continual Learning (CL) techniques in multiple sub-tasks setting for bug localization (each of which operates on either stationary or non-stationary data), comparing it against a bug localization technique that leverages the BERT model, a deep reinforcement learning-based technique that leverages the A2C algorithm, and a DL-based function-level interaction model for semantic bug localization. Additionally, we enhanced the CL techniques by using logistic regression to identify and integrate the most significant bug-inducing factors. Our empirical evaluation across seven widely used software projects shows that CL techniques perform better than DL-based techniques by up to 61% in terms of Mean Reciprocal Rank (MRR), 44% in terms of Mean Average Precision (MAP), 83% in terms of top@1, 56% in terms of top@5, and 66% in terms of top@10 metrics in non-stationary setting. Further, we show that the CL techniques we studied are effective at localizing changesets relevant to a bug report while being able to mitigate catastrophic forgetting across the studied tasks and require up to 5x less computational effort during training. Our findings demonstrate the potential of adopting CL for bug localization in non-stationary settings, and we hope it helps to improve bug localization activities in Software Engineering using CL techniques.

==> extra_content.tex <==
Introduction:

\Amin{sound like background to me, just mention the-state-of-the-art techniques, and then the research gap/problem we want to cover}Bug localization is a largely adopted process by developers aiming to find the root cause of a bug and relevant software artifacts that need to be fixed based on a given report \cite{liang2022modeling}. However, such a process is challenging as it requires familiarity with the target software systems and the relevant software artifacts associated with the bug \cite{bacchelli2013expectations}. Researchers have proposed numerous bug localization techniques ~\cite{zhou2012should,liang2022modeling,chakraborty2023rlocator,moser2008comparative,chidamber1994metrics,antoniol2005feature}. Specifically about Machine Learning (ML) techniques, prior studies leveraged ML by training models, e.g., Convolutional Neural Network (CNN) and Recurrent Neural Network (RNN) to locate bugs at the changeset-files (i.e., a collection of source code files that were modified as part of a particular commit) level~\cite{xiao2018machine,liang2019deep}. These techniques measure the cosine similarity between bug reports and changeset-files and rank the files based on their similarity score. 
%Liang et al. \cite{liang2022modeling} fine-tuned a language model to learn semantic relations between source code files and bug reports. The model outputs semantics features related to the bug report and the source code files to feed them to a learn-to-rank model. 
Liang et al. \cite{liang2022modeling} went beyond by exploring the semantic relations between source code and bug reports.
For that, they fine-tuned a language model to output semantic features that are fed as input to a learn-to-rank model.
%Next, the learn-to-rank model outputs the relevance between the bug report and the source code files. 
Chakraborty et al.~\cite{chakraborty2023rlocator} used Deep Reinforcement Learning (DRL) to locate buggy changeset-files by training an agent to pick buggy changeset-files based on their relevance to a bug report and the distance between the already picked changeset-files. 

The Atari suite environments \cite{mnih2013playing} consist of a wide range of environments, each with unique dynamics, rules, and objectives. As the CL agent moves from one environment to another, the distribution of the state-action pairs it experiences can shift significantly. This change in the environment represents concept drift, where the agent needs to adapt to new situations that were not present in its previous learning phase. During the evaluation of each studied environment (i.e., each environment that was involved during the training cycle), the CL agents showed similar performance compared to agents that are trained separately on the studied environment, effectively addressing data distribution shift and improving training cost compared to training on each environment separately.
